Continual Learning with Self-Organizing Maps

Despite remarkable successes achieved by modern neural networks in a wide range of applications, these networks perform best in domain-specific stationary environments where they are trained only once on large-scale controlled data repositories. When exposed to non-stationary learning environments, current neural networks tend to forget what they had previously learned, a phenomena known as catastrophic forgetting. Most previous approaches to this problem rely on memory replay buffers which store samples from previously learned tasks, and use them to regularize the learning on new ones. This approach suffers from the important disadvantage of not scaling well to real-life problems in which the memory requirements become enormous. We propose a memoryless method that combines standard supervised neural networks with self-organizing maps to solve the continual learning problem. The role of the self-organizing map is to adaptively cluster the inputs into appropriate task contexts - without explicit labels - and allocate network resources accordingly. Thus, it selectively routes the inputs in accord with previous experience, ensuring that past learning is maintained and does not interfere with current learning. Out method is intuitive, memoryless, and performs on par with current state-of-the-art approaches on standard benchmarks.

==> sec_intro.tex <==
 %to add: discussion of existing online adaptive network methods, like dynamic execution, bandit-based representation selection, routing nets and more recent extensions of those by Sergey Levine and others; defining different types of  lifelong learning scenarios.

\section{Introduction}
\vspace{-0.1in}
Learning algorithms typically operate on the entire training data set, in an offline mode, and may require costly re-training from scratch when new data becomes available. In contrast, humans learn continuously ("online"), adapting to the environment while leveraging past experiences. In this setting of {\em continual} learning, an agent is presented with a stream of samples (input-output pairs) from a non-stationary data distribution, such as a sequence of different classification tasks.
%The data distribution may change when switching from one task to another.
The agent has to learn the input-output relationships associated with different data distributions in order to be able to adapt well to new tasks without forgetting the tasks learned previously, i.e. to avoid the {\em catastrophic forgetting} \cite{catastrophic} problem in continual learning. Several types of approaches to this problem have been proposed in the past that introduce structural robustness \cite{goodfellow2013,srivastava2013}, regularize the parameters \cite{yosinski,Zenke2017,ewc} or utilize memory buffers \cite{gem,mbpa}. While the memory-based methods are among the most successful methods, these approaches generally utilize explicit task labels when storing instances of past learning and they also don't scale well to real life problems.

%improving  structural robustness to forgetting using specific nonlinearities %\cite{srivastava2013}, or injecting noise \cite{goodfellow2013};  introducing %constraints, e.g., selectively freezing some of the network parameters, reducing the %learning rate \cite{razavian, yosinski}, or encouraging the weights to remain close to %previous values \cite{Zenke2017,ewc};  or using memory of some previous samples  %\cite{gem,mbpa}. However, these methods typically rely on storing some of the previously %encountered samples, and often require an explicit indication of when the task switching %occured.
%\todo{why are these methods not sufficient?}.
%\todo{if we have space, we might want to write a bit about catastrophic forgetting here}

% %Problem of continual learning has been thought about since ??, and it has attracted more attention in the recent years. 
% Several approaches have been proposed to tackle  catastrophic forgetting \cite{catastrophic} in continual learning.
% They can roughly be divided into three classes. 
% (i) structural robustness: these methods make use of structural elements in the network to make the network robust to forgetting. Use of specific nonlinearities \cite{srivastava2013}, or injecting noise \cite{goodfellow2013} have previously been used. 
% (ii) parameter regularization: these methods reduce interference by setting up constraints on parameters of the network. Constraints include selectively freezing some of the network parameters, reducing the learning rate \cite{razavian, yosinski}, or encouraging the weights to remain close to previous values \cite{Zenke2017,ewc}. 
% (iii) memory-based methods: several studies have proposed augmenting the learning objective with "sample memory buffers" to help to remember the previously learned tasks \cite{gem,mbpa}.\todo{if we list all these methods, we need to reason why we do not test against them here. Maybe we don't have to include an extended list of all methods here, given 4 page limit.}

% We consider supervised continual learning problem, where a learning  agent is presented with  a stream of labeled samples (input-output pairs) coming from some  nonstationary data distribution, produced, for example, by a  sequence of different classification tasks; the data distribution may change either gradually or abruptly when switching from one task to another. The objective is to learn the input-output relationships associated with different tasks, or data distributions, so that the model can adapt well to the new tasks while not forgetting the tasks learned previously.

Herein, we propose to capture the essence of the multimodal data distributions encountered in continual learning via the unsupervised learning mechanism known as Self-Organizing Map (SOM).  The map learns simultaneously with a supervised feedforward neural net in such a way that the SOM routes each input sample to the most relevant part of the network.  Unlike previous methods, SOMs do not require explicit information about the change in task, or an explicit memory of previous samples, while still achieving performance levels close to the current state-of-art on several benchmarks.
%The per-task network relevance map is learned without supervision and inherently adapts to new data distributions, while the task-specific input-output mappings are learned with supervised backpropagation.
%This approach achieves state-of-the-art \todo{can we claim SOTA? are we within the error bars? or say "is close to SOTA"?} %performance, but unlike current algorithms, does not depend on a memory of samples.

%Role of the continual learning algorithm is to allow the agent to learn all the correspondences between input-output pairs as they are experienced sequentially. 
%In order to allow this, our proposed algorithm learns to assign resources for learning each data point based on the likelihood of observed sample belonging to each distribution (i.e. as a form of routing in the network) [??ref].
%We adopted Self-Organizing feature Maps (SOM) in conjunction with supervised learning with back-propagation to allow the network to automatically select subparts of the network when facing different tasks sequentially. 
 
\begin{comment}
\section{Continual Learning}
\todo{I moved this away from the intro, I wouldn't start with full-on abstract variables. We first need to motivate why any of this is relevant.
I'm also not sure how this connects to our methods later in the text, so unless the mathematical setup here is useful for algorithms later on, I'd cut it for now (but perhaps re-use in a full paper)}
In the  classical {\em offline supervised learning} setting, a learning agent is given a fixed training data set $D_{tr}=\{(\bs{x}_i,y_i)\}^n_{i=1}$ of $n$ samples, each containing an input  feature vector $\bs{x}_i \in \cal{X}$  associated with the corresponding output (target, or label) $y_i \in \cal{Y}$; training samples are usually  assumed to be i.i.d. and belong to the same joint probability distribution $P(\bs{x},y)$. The learning task is often formulated as a {\em function approximation} problem, i.e. finding a function, or model, $f(\bs{x}|\bs{\theta}): \cal{X} \rightarrow \cal{Y} $ from a given class of models (e.g.,  neural networks) where  $\bs{\theta}$ are the parameters estimated from data.
Given a loss function $l(f(\bs{x}),y|\bs{\theta})$, the parameter estimation is formulated as an empirical risk minimization (or, similarly,  maximum likelihood estimation) problem:  $\min_{\bs{\theta}}\sum_{(\bs{x}_i,y_i) \in D_{tr} } l(f(\bs{x}),y|\bs{\theta})$.

On the contrary, {\em online learning }  assumes no fixed training dataset but rather a stream of data samples, where   unlabeled feature vectors arrive one at a time, or in small mini-batches, and the learner must   assign the labels to those inputs, receive the correct labels, and   update the model accordingly, in iterative fashion. While classical online learning assumes i.i.d. samples, the {\em continual}, or {\em lifelong learning} does not make such assumption, and requires a learning agent to handle non-stationary data streams. A common setting (e.g., \cite{gem}) is a sequence of different datasets associated with  different classification tasks. 

%\begin{comment}
%The standard problem of supervised learning is formulated as follows. Let $\bs{D^{tr}} = \{ (\bs{x}_i,y_i)|i=1,...,N, (\bs{x}_i,y_i)  \in \cal{X} \times \cal{Y} \}$ be a set of labeled training samples, typically assumed to be i.i.d. and come from the same joint probability distribution $P(\bs{x},y)$, where $y_i \in C$ are class labels, $C=\{0,…,m\} $ in case of discrete classification problems (e.g., binary when m=1), and $C=R$ in case of continuous regression problems. In deterministic supervised classification problem it is assumed that the class label $y$ is a function of the input $\bs{x}$, $y=f(\bs{x})$, whether deterministic, or probabilistic, in probabilistic classification setting; learning is formulated as a {\em function approximation} task. Namely, a family $M$ of classification  models, such as linear regression models, decision trees, deep neural networks, or any other type, is assumed, where each model with parameters $\bs{\theta}$ represents a function $f_M(\bs{x}|\bs{\theta}): \mathbb{R}^m \rightarrow C $, and learning involves finding a set of parameters $\bs{\theta}$, defining a function (model) in $M$ which minimizes the empirical risk, i.e. average error, over the set of {\em test samples} $(\bs{D^{test}} = \{ (\bs{x}_1,y_1) \cdots, (\bs{x}_n,y_n) \in \mathbb{R}^m \times C \}$:
%\begin{eqnarray}
%E_{D^{test}} = \sum_{i=1}^n 1(f_M(\bs{x_i}) = f(\bs{x_i}))
%\end{eqnarray}

%The continual learning problem is can be  defined in several ways, but we will define it here as follows.
\end{comment}

==> sec_methods.tex <==
\vspace{-0.1in}
\section{Self-Organizing Maps for Continual Learning}
\vspace{-0.1in}

% \begin{figure}
%   \begin{minipage}[c]{0.45\textwidth}
%     \includegraphics[width=\textwidth]{figures/som_overview.pdf}
%   \end{minipage}\hfill
%   \begin{minipage}[c]{0.3\textwidth}
%     \caption{
%       caption
%     }
%   \end{minipage}
% \end{figure}

% \begin{figure}
% \floatbox[{\capbeside\thisfloatsetup{capbesideposition={left,top},capbesidewidth==.5\textwidth}}]{figure}[\FBwidth]
% {\caption{A test figure with its caption side by side}\label{fig:test}}
% {\includegraphics[width=.5\textwidth]{figures/som_overview.pdf}}
% \end{figure}

%
\begin{wrapfigure}{R}{0.38\textwidth}
  \vspace{-0.25in}
  \begin{center}
    \includegraphics[height=1.6in,width=.38\textwidth]{figures/som_overview.pdf}
  \end{center}
  \caption{\textbf{SOMLP setup.} 
  Red borders indicate supervised training; SOM is trained in an unsupervised manner.
%   Our network consists of two fully-connected layers (trained with supervision, red border). The SOM layer is positioned in parallel to the hidden layer and learns a topographical mapping of the input space onto network nodes without supervision (dashed line).
%   %The dashed line and the colored dots demonstrates the correspondence between nodes in the FC-layer and the SOM. 
%   Output of the SOM is multiplied to the hidden-layer output before being fed to the second layer. 
%   %Red border lines highlight parts of the network that are trained supervised.
  }
  \label{fig_som_setup}
  \vspace{-0.12in}
\end{wrapfigure}
%

Self-Organizing Maps (SOMs) \cite{Kohonen1990} are a type of artificial neural network which reduce the input from a high-dimensional ($N$) space to a low-dimensional representation without supervision.
%Self-Organizing Maps (SOMs) are a type of artificial neural network performing unsupervised dimensionality reduction, as it is trained to produce a low-dimensional representation of the $N$-dimensional input space. 
Unlike supervised training via error-correction (backpropagation), self-organizing maps employ unsupervised competitive learning in order to map similar input vectors to physically nearby nodes in the map layer.
%aiming to preserve the topological properties of the input space.
%Unlike supervised feedforward networks trained via error-correcting learning (backpropagation),  self-organizing maps use unsupervised  competitive learning, while aiming to preserve the  topological properties of the input space.
Namely, each SOM node will be associated with an $N$-dimensional weight vector, and, at each iteration,  the next input sample will be assigned to  the most similar network node called  the Best Matching Unit (BMU). Trainable weights associated with the BMU along with weights of its topographical neighbors (determined by neighborhood radius $\sigma$) are tuned to reduce the error between the weights and the input, (proportioanl to a learning rate $\alpha$) so that the neighborhood becomes more similar to the input. 
This allows the SOM to only adapt parts of its parameters in response to each observed input. To stabilize the learning, both $\alpha$ and $\sigma$ parameters are decayed during learning (with an exponential decaying rate of $\tau$).

SOMs has been previously used as a potential solution to the catastrophic forgetting problem \cite{Gepperth2016} but it has been shown that the proposed algorithms often fail on small-scale benchmarks like MNIST-permutations and rotations \cite{Kemker2017}. Here we introduce the Self-Organized Multi-Layer Perceptron (SOMLP) where a SOM layer is used in parallel with a fully-connected layer, as illustrated in \Cref{fig_som_setup}.
%In our proposed method, we use a SOM layer in parallel with a fully connected layer, named Self-Organized MultiLayer Perceptron (SOMLP) as illustrated in \Cref{fig_som_setup}. 
% SOM weights are randomly initialized
The SOM receives the same input as the fully-connected layer and is trained without supervision on the network inputs (\Cref{alg_som}). During the training it learns the input distribution for each task and, most importantly, a 2D map of relationships between the tasks. 
For every input, an output mask $\Gamma$ is computed based on the Euclidean distances between the input and SOM weight vectors, as shown in \Cref{alg_som} (tuned with hyperparameter $\epsilon$), and is multiplied with the output of the fully connected layer (\Cref{fig_som_setup}).
This allows the network to allocate resources (i.e. nodes) to learning input-output associations for each task, and mask irrelevant nodes. In addition, the SOM shares nodes between similar tasks while using separate nodes for dissimilar tasks. 
The overall training procedure is shown in \Cref{alg_training}, which includes the option of pretraining SOM weights on unlabeled data from different tasks (if available).  


%\begin{small}
\begin{figure}[h]
\begin{minipage}[t]{.48\textwidth}
  \null
  \begin{algorithm}[H]
    \caption{SOM update}
    \label{alg_som}
    \begin{algorithmic}[1]
        \GIVEN input $x$ and SOM weights $\theta$ at step $t$, nodes coordinate matrix $L$, batch size $N_{bs}$, number of nodes $N_n$, %total number of steps $N_{s}$, %commented out since it does not seem to be used later
        and hyperparameters $\alpha,\sigma,\epsilon,\tau$.
        
        
        \STATE $\Bar{x} = \frac{1}{N_{bs}}\sum_{i\in batch}^{N_{bs}}{x_i} ~~$ \Comment{average  over batch}
        
        \LineComment{Find best matching unit (BMU) for $\Bar{x}$ } 
        
        \STATE $i^*=argmin_i(\norm{\Bar{x}-\theta_i})$
        
        \STATE {\bfseries }\textbf{for } $i = 1, 2, . . . ,N_{n}$ \textbf{do} \Comment{compute}
        \STATE \quad $D_{i} = \norm{L_{i} - L_{i^*}}$  \Comment{distances to BMU}
        \STATE {\bfseries } \textbf{end} 
        \STATE $\phi = e^{D/\sigma^2}$\Comment{neighborhood mask}  
        \STATE $\Gamma=e^{-\norm{x-\theta}/\epsilon}$ \Comment{output mask}
        
        \STATE $\alpha \leftarrow \alpha e^{-\tau t /N_{steps}}$ \Comment{Adjust $\sigma$ and $\alpha$}
        \STATE $\sigma \leftarrow \sigma e^{-\tau t /N_{steps}}$
        \STATE $\theta_i \leftarrow \theta_i + \alpha \phi (x-\theta_i)$  \Comment{Update weights }
        
    \end{algorithmic}
  \end{algorithm}
\end{minipage}%
\hfill
\begin{minipage}[t]{.48\textwidth}
  \null
  \begin{algorithm}[H]
    \caption{Training procedure}
    \label{alg_training}
    \begin{algorithmic}[1]
    \GIVEN   Training datasets $(X_{t}, Y_{t})$ for each task $t$ out of $N_T$ tasks, and   data subsets $(X^{pr}_{t}, Y^{pr}_{t})$ available for SOM pretraining.
    \INITIALIZE SOM and MLP weights randomly.
     
    \LineComment{Pretrain sequentially w/ unlabeled data} % sequentially}
    \STATE {\bfseries }\textbf{for } $t = 1, 2, . . . ,N_{T}$ \textbf{do}
    \STATE \quad {\bfseries }\textbf{for } batch in $ X^{pr}_{t}$ \textbf{do}
    \STATE \quad \quad Update SOM weights using Alg. \ref{alg_som}
    \STATE {\bfseries }\quad \textbf{end}
    \STATE {\bfseries } \textbf{end}
     
    \LineComment{Train sequentially using labeled data}
    \STATE {\bfseries }\textbf{for } $t = 1, 2, . . . ,N_{T}$ \textbf{do}
    \STATE \quad {\bfseries }\textbf{for } batch in $ (X_{t}, Y_{t})$ \textbf{do}
    \STATE \quad \quad Update SOM weights using Alg. \ref{alg_som}
    \STATE \quad \quad Update MLP weights using SGD
    \STATE {\bfseries }\quad \textbf{end}
    \STATE {\bfseries } \textbf{end}
    \end{algorithmic}
  \end{algorithm}
\end{minipage}
\end{figure}
%\end{small}


==> sec_results.tex <==
\vspace{-0.1in}
\section{Experiments}
\vspace{-0.1in}
We evaluated SOMLP against three other baseline methods: a naive Multi-Layer Perceptron (MLP), Elastic Weight Consolidation (EWC) \cite{ewc} and Gradient Episodic Memory (GEM) \cite{gem}. We evaluated all methods on two standard benchmark datasets, \emph{MNIST-permutations} and \emph{MNIST-rotations} \cite{gem}. 
MNIST-permutations consists of 20 random pixel permutations of the standard MNIST dataset while MNIST-rotations contains 20 rotations of MNIST digits between 0 and 180 degrees. 

All experiments were performed on a fully-connected network with a single hidden layer with $n_{h1}$ units, varying across the experiments,  % of size 1600 
and an output layer with $n_{h2} = 10$ units. % ($n_{h1}=1600$, $n_{h2}=10$). 
For SOMLP, the hidden layer is augmented with a SOM of the same size and the output of $n_{h1}$ is multiplied by the SOM output before being fed to the next layer.
For a fair comparison with respect to the numbers of parameters, we used $n_{h1} = 3200$ for MLP, EWC and GEM and $n_{h1} = 1600$ for SOMLP\footnote{The total number of parameters for MLP, EWC and GEM is $2,540,800 = 3200 \times 784 + 3200 \times 10$; and for SOMLP $2,524,800 = 1600 \times 2 \times 784 + 1600 \times 10$}.
%We observed that having a large number of units $n_{h1}$ is  necessary for SOMLP's good performance, as it needs  to build a large enough map; this can be a potential limitation of our current approach, since, in comparison, EWC and GEM already work well with $n_{h1} = 100$.

All networks were trained for 1 epoch on the training set, learning 20 tasks in sequence. 
For each task, the network is presented with 60,000 samples. The   hyperparameter settings used in the experiments are summarized in supplementary \Cref{table_hyperparameters}.

In addition, EWC and GEM methods require additional memory slots.
EWC uses a memory buffer to save samples before computing the Fisher matrix before moving to the next task. On the other hand,
GEM uses a memory buffer per task to retain samples for experience replay.
A scalar "memory strength" additionally dictates how much to weigh previous samples.
In our experiments, we varied the number of memory slots between 8 to 5120 for EWC with a memory strength of 3, and 256 to 5120 for GEM with a memory strength of 0.5.
An advantage of SOMLP is that it does not require a sample memory buffer.

In our approach, we used two methods for pretraining SOM weights. The first one pretrains the weights on the unlabeled MNIST training set, with large neighborhood values ($\textnormal{SOMLP}_s$), while for the second one, the weights are pretrained on 10\% of the training set from all the tasks in the benchmark ($\textnormal{SOMLP}_m$). We only use the input images for pretraining. 

\vspace{-0.1in}
\section{Results}
\vspace{-0.1in}

\Cref{table_perfs} shows the networks' performances on each benchmark dataset after learning a battery of 20 tasks.
%
\begin{table}[bh]
\begin{center}
\begin{small}
    \caption{Comparison of average performances on benchmark datasets. Number of parameters in each network were matched by changing the network size.}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c}
    \toprule
    \label{table_perfs}
    \textbf{Network} & \textbf{Memory Size} & \textbf{\#Parameters (M)} & \textbf{\begin{tabular}[c]{@{}c@{}}Performance (\%)\\ (MNIST-Permutations)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Performance (\%)\\ (MNIST-Rotations)\end{tabular}} \\
    \midrule
    MLP              & 0                 & 2.5           & 29$\pm$0.6                           & 64.4$\pm$0.4         \\
    EWC-Low Mem      & 8                  & 2.5           & 84.8                              & 59.1             \\
    EWC-High Mem     & 5120             & 2.5           & 83.6                                 & 49.8             \\
    GEM-Low Mem      & 320                 & 2.5           & 68.3                             & 71.5             \\
    GEM-High Mem     & 5120            & 2.5                  & 93.3                           & 92.6             \\
    $\textnormal{SOMLP}_s$         & 0         & 2.5          & 65.9$\pm$5.2                      & 59.1$\pm$6.6         \\
    $\textnormal{SOMLP}_m$      & 0         & 2.5          & 85.4$\pm$1.8                      & 79.1$\pm$0.8      \\
    \bottomrule
    \end{tabular}}
    \end{small}
\end{center}
\end{table}
%
On MNIST-permutations, $\textnormal{SOMLP}_m$ performed on par with EWC but lower than GEM with large memory buffers, whereas it outperformed EWC on MNIST-rotations but still was lower than GEM. On the other hand, in the low-memory case that the size of available memory is reduced, $\textnormal{SOMLP}_m$ performs better than all baseline methods. In contrast, $\textnormal{SOMLP}_s$ only performed better than EWC on MNIST-rotations. Naive MLP worked fairly well on MNIST-rotations but lower than all methods on MNIST-permutations.

%, "SOMLP" performed lower than both GEM and EWC methods with 5120 and 16 sample memory slots. In contrast, "SOMLP-pretrain" performed better than EWC but worse than GEM. 
%Overall, we found that on both benchmarks, "SOMLP" performed lower than both GEM and EWC methods with 5120 and 16 sample memory slots. In contrast, "SOMLP-pretrain" performed better than EWC but worse than GEM. 
%All baseline methods performed better that the SOM variants on the first task partly because of the larger network size in these methods. %\todo{how do we know this? - just observed and }. 

\begin{figure}[t]
\center
\includegraphics[width=\linewidth]{figures/memories.pdf}
\caption{\textbf{Sample memory size effect on performance.}
Both GEM and EWC depend on the right amount of memory.
For GEM, more memory generally leads to better performance, whereas the optimal EWC memory size seems to depend on the dataset.
SOMLP does not require sample memory.
}
\label{fig_mem}
\end{figure}
\begin{figure}[h]
\center
\includegraphics[width=.7\linewidth]{figures/som_masks.pdf}
\caption{\textbf{Learned SOM.}
(left) Euclidean distance between SOM nodes for each benchmark during a single run. (right) SOM masks found for different tasks during a single run on each benchmark.}
\label{fig_masks}
\end{figure}

It should be noted that both EWC and GEM make use of a "sample memory buffer" as well as explicit information about when the task is switched while SOMLP requires neither a memory buffer nor knowledge of task switching.
We examined the effect of the amount of sample memory on mean performance\footnote{We note that EWC additionally stores the Fisher matrix associated with each task which we did not account for in our memory requirement estimate.}. 
We found that the performance of GEM on both benchmarks is significantly reduced with smaller memory sizes. EWC performance is almost constant in the MNIST-permutations benchmark and even decreases with enlarged memory buffer in MNIST-rotations (\Cref{fig_mem}). 

We also examined the mean performance during sequential learning of all tasks (\Cref{fig_pertask}) on each dataset. As more tasks are learned, EWC and $\textnormal{SOMLP}_s$ experience some degree of forgetting and therefore the mean performance decreases with more tasks. While both GEM and $\textnormal{SOMLP}_m$ are able to maintain the same level of mean performance throughout, $\textnormal{SOMLP}_m$ is consistently below GEM's level of performance. This is potentially due to lower network capacity in our SOMLP approach because of (1) smaller network size and (2) per-task SOM masks that limits the resources available to learn each task. 

The learned feature maps and per-task masks for each benchmark are shown in \Cref{fig_masks}. 
In MNIST-permutations, because of the random pixel permutations in each task, masks corresponding to each task are independent of each other. Conversely, in MNIST-rotations, the learned masks share nodes between tasks that are more similar (i.e. slightly rotated tasks) and use independent nodes for more dissimilar tasks (e.g. tasks that are separated by larger rotation angles).


%\section{Conclusion}
% Our results are significant because:\todo{this needs work.}

% \begin{enumerate}
%     \item Unlike in most previous algorithms, that need to be informed about task id in order to manage their memory buffers, our proposed method is completely independent of that information. While this might be considered as a minimal usage, it should be pointed out that lack of this information could only be resolved by having very strong assumptions on equality of the number of samples corresponding to each task. 
%     \item SOM-augmented networks are cheap to train and evaluate and they are easily scalable. [?? need some numbers here as ref??]
% \end{enumerate}

% On another note, as we mentioned earlier the utility of SOM layer is dependent on its weights initialization. We also experimented with allowing the network to be pretrained on all or part ($\sim$10\%) of the samples from the training set of all tasks. Allowing this form of pretraining significantly elevated the performance of our method in learning without forgetting.
% [??justify why this is plausible]

% The main advantage of our proposed method is that it does not have a memory component and it is fast to compute compared to previously proposed methods like \cite{ewc,gem}. 


% SOM requires no task knowledge
% Both EWC and GEM utilize information about the current task: EWC computes the Fisher matrix when the task switches and GEM stores memory per task.




% %


% TODO
% seems like it's really the memory that is slowing GEM down. the first 10% of data are done in half an hour, but the more tasks, the more it slows down. another thing to highlight % for the full paper, it doesn't scale with increased memory demands

